CBLUE: A Chinese Biomedical Language Understanding Evaluation Benchmark

Artificial Intelligence (AI), along with the recent progress in biomedical language understanding, is gradually changing medical practice. With the development of biomedical language understanding benchmarks, AI applications are widely used in the medical field. However, most benchmarks are limited to English, which makes it challenging to replicate many of the successes in English for other languages. To facilitate research in this direction, we collect real-world biomedical data and present the first Chinese Biomedical Language Understanding Evaluation (CBLUE) benchmark: a collection of natural language understanding tasks including named entity recognition, information extraction, clinical diagnosis normalization, single-sentence/sentence-pair classification, and an associated online platform for model evaluation, comparison, and analysis. To establish evaluation on these tasks, we report empirical results with the current 11 pre-trained Chinese models, and experimental results show that state-of-the-art neural models perform by far worse than the human ceiling. Our benchmark is released at \url{https://tianchi.aliyun.com/dataset/dataDetail?dataId=95414&lang=en-us}.

==> tables/ee_badcase.tex <==
\begin{CJK*}{UTF8}{gbsn}
\begin{table}[t]
  \label{tab:ee_badcase}
  \centering
 % \resizebox{\textwidth}{!}{
  \begin{tabular}{p{5.6cm}p{3cm}ccc}
    \toprule
    {\textbf{Sentence}} &
    {\textbf{Word}} &
    {\textbf{Label}} & 
    {\textbf{RO}} & 
    {\textbf{MB}} \\
    \midrule
    血液生化分析的结果显示维生素B缺乏率约为12\%～19\%。& 血液生化分析 & Ite & Pro & Pro\\
    The results of blood biochemical analysis show that vitamin B lack rate is about 12\% to 19\%. & blood biochemical analysis & Ite & Pro & Pro\\
    \midrule
    皮疹可因宿主产生特异性的抗毒素抗体而减少。 & 抗毒素抗体 & Bod & O & Bod\\
    The rash can be reduced by the host producing specific anti-toxin antibodies. & anti-toxin antibodies & Bod & O & Bod \\
    \midrule
    饮食控制、锻炼或口服降糖药治疗有效。 & 口服降糖药 & Pro & O & O\\
    Diet control, exercise or oral hypoglycemic treatment effective. &  oral hypoglycemic & Pro & O & O \\
    \midrule
    根据遗传物质的结构和功能改变的不同，可将遗传病分为五类：1.染色体病指染色体数目异常，或者染色体结构异常，包括缺失、易位、倒位等 & 缺失, 易位, 倒位 & Sym, Sym, Sym & O & Sym, Sym, Sym\\
    According to the structure and function of genetic material, genetic diseases are divided into five categories: 1. Chromosomal diseases refer to abnormal chromosome number or chromosome structure abnormalities, including deletions, translocations, inversions... &  deletions, translocations, inversions & Sym, Sym, Sym & O & Sym, Sym, Sym\\
    \bottomrule
  \end{tabular}
  %}
  \caption{The CMedEE diagnostics: We evaluate roberta-wwm-ext and PCL-MedBERT on 3 representative sentences, with their gold labels and model predictions. Ite(medical test items), Pro(medical procedure), Bod(body) and Sym(clinical symptoms) are labels for medical named words. O means that the model fails to extract the entity from sentences. RO=roberta-wwm-ext, MB=PCL-MedBERT.}
  \label{cmedee}
\end{table}
\end{CJK*}
 
% \begin{tabular}[c]annotator 3\\ 234\end{tabular}
% \begin{CJK*}{UTF8}{gbsn}
% \end{CJK*}
